Object-Centric Multi-View Aggregation

We present an approach for aggregating a sparse set of views of an object in order to compute a semi-implicit 3D representation in the form of a volumetric feature grid. Key to our approach is an object-centric canonical 3D coordinate system into which views can be lifted, without explicit camera pose estimation, and then combined -- in a manner that can accommodate a variable number of views and is view order independent. We show that computing a symmetry-aware mapping from pixels to the canonical coordinate system allows us to better propagate information to unseen regions, as well as to robustly overcome pose ambiguities during inference. Our aggregate representation enables us to perform 3D inference tasks like volumetric reconstruction and novel view synthesis, and we use these tasks to demonstrate the benefits of our aggregation approach as compared to implicit or camera-centric alternatives.

==> intro.tex <==
\section{Introduction}

A central problem in computer vision is to recover the 3D structure of the world from 2D views of it, namely images. In this work we focus on the single-object setting: how to recover 3D information from one or more views of an object. By ``3D information’’ we do not necessarily mean traditional 3D reconstruction but more generally the ability to execute a plethora of tasks that an agent interacting with the object in the 3D world might find useful. Such tasks can include new view generation, collision detection, dimension/size estimation, etc. Of course, a full 3D reconstruction provides a representation that subsumes all these tasks but it is not always required or possible.

Classical approaches such a Structure from Motion (SfM) focus on the setting where many views (say tens to hundreds) are available so that geometric correspondences between them can be used to infer camera pose and induce 3D structure \cite{tomasi1992shape,koenderink1991affine}. More recently there has been a flurry of activity on object reconstruction from a single view, exploiting machine learning and especially deep learning approaches to resolve depth and hallucinate information invisible in that view \cite{choy20163d,fan2017point,tulsiani2017multi}, building on large 3D model repositories such as ShapeNet \cite{chang2015shapenet} for training. Our work falls in between these two extremes and addresses situations where only a few views (say one to four) \todo{OL: this is in-fact a useful scenario encountered in marketplace websites...should we say something about it?} of an object are available and need to be aggregated for 3D inference. While a number of the prior single view reconstruction methods can also benefit from the incorporation of additional views, the aggregation process itself has not been dealt in fully satisfactory manner (for example, to guarantee order-independence in the view aggregation process \todo{OL: or to deal with unknown viewpoint}).

If the class of the object can be inferred from the view and we have many example instances of this class as 3D models, then we can try to interpret the given object view in the context of this prior knowledge. For example, when placed in a canonical pose, many airplanes have the same overall 3D shape structure consisting of a long ellipsoidal fuselage and roughly planar wings orthogonal to the fuselage. Thus we can imagine a canonical bounding volume for airplanes with a class-specific priors for where different parts go. We can then try to ``lift’’ the views of the actual airplane we see and place them into that canonical space using object-centric as opposed to world coordinates. This is the approach we follow in this paper, inspired by the NOCS (normalized object coordinate space) formulation of \cite{wang2019normalized}. Unlike more traditional computer vision techniques that are camera-focused and need to know or estimate the camera pose for each view in a world coordinate system so as to properly integrate them, we instead accomplish view aggregation without explicit camera pose estimation, by directly lifting views into an object-centric (in this case ``airplane'') space.

A major design choice here is how explicit to make the 3D representation. This can vary from using just a single latent vector to represent the object (where 3D is entirely implicit) to a traditional fully explicit 3D representation, such as a mesh. We have recently seen successes in using semi-implicit representations, such as the DeepVoxels work \cite{sitzmanndeepvoxels} that combine a 3D voxel grid with an implicit latent vector in each voxel coding the contents of that cell (many more such hybrid designs seem possible). The advantage of a hybrid representation is that it is still end-to-end trainable for one or more downstream tasks (e.g., new view generation), while also accommodating variations within a task (e.g., which view to generate) that benefit from explicit 3D information such as depth ordering or occlusion information. For the same reasons, we also adopt a similar semi-implicit representation from which both a voxelized fully explicit representation 3D can be generated, as well as arbitrary 2D views, on demand.

Our object-centric approach allows further exploitation of prior object knowledge that is difficult to incorporate in camera-centric approaches. For example, many objects possess important symmetries that can be inferred from knowledge of the object class and the observed view or views. With such knowledge, when we lift a given view into the canonical object-centric space in 3D, we can augment the observed regions by their inferred symmetric counterparts, effectively enhancing our understanding of the 3D structure of the object and allowing us to produce a complete 3D representation from fewer views. There are a number of subtle but important effects of this symmetry augmentation in our network design. One is that symmetry augmentation is likely to yield sharper reconstruction of occluded geometry than direct prediction of that geometry in the network. This is because direct reconstruction can suffer from the high-frequency filtering commonly seen in autoencoders -- while we predict much lower dimensional objects, symmetry transforms, which then effectively copy predictions from detailed visible geometry, preserving local information. A second important effect is that symmetry augmentation also solves the problem of pose ambiguities due to object symmetries or part occlusions (e.g., a coffee cup whose handle is invisible in the view) -- by effectively generating in the object coordinate space the union of the lift from all possible valid poses, thus making such ambiguities immaterial.

Our overall architecture consists of three parts: a) a network that takes a single view image and lifts it into a semi-implicit representation of the seen object in a voxelized object-centric 3D space annotated with learned features per voxel, b) a symmetric view aggregator that can combine a variable number of lifts from different views into a single semi-implicit representation, and c) networks that then use this representation for different downstream tasks, such as voxelized 3D reconstruction or novel view synthesis. Note that our design can deal with an arbitrary and variable number of input views and the resulting representation is independent of the order in which the views are provided/aggregated, unlike sequential approaches based on RNNs or LSTMs \cite{choy20163d}.

In summary, we show how to work in the few view realm and infer 3D information useful for a variety of tasks. Our key contributions are:
\bitem
    \item by using an object-centric coordinate system we obviate the need for camera pose estimation in 3D inference and view aggregation
    \item our symmetry-aware view lifting into the object-centric space allows us to extract more information from each view, infer more detail in unseen areas, and bypasses the challenges raised by ambiguous view poses
    \item our aggregation mechanism is able to incorporate a variable number of views and is order independent
    \item our semi-implicit 3D representation carries a strong geometric inductive bias in its formulation, combining latent local elements that that can be trained in an end-to-end fashion, while also adhering to an underlying object-centric 3D space that makes it flexible and adaptable for multiple downstream tasks. 
\eitem

%order invariance of aggregation.

%use of symmetry vs. direct prediction -- why is predicting the predictor better than predicting?

%quantifying reconstruction and view quality. dependence of quality on the number of views.

%motivate the setup. say there are two approaches to multi-image aggregation. classical ones  explicitly construct 3D volumes or point clouds via feature matching, but require many images. Introduce `multi-image' vs `multi-view' setups, say we tackle `multi-image' settings. Learning based methods to do so \eg 3D-R2N2 are completely implicit and ignore the geometry of the problem.

%Some approaches aim to integrate the benefits of geometry and learning \eg LSM, but crucially rely on privileged information like known camera views to do so.



==> tables/pred3d.tex <==
\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{5pt}
\begin{table}[htb!]
\centering
\vspace{0pt}
\centering
\footnotesize
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{lccccccccccccc|c}
    \toprule
    \textbf{Classes}     &  \textbf{aero}     &  \textbf{bench}     &  \textbf{cabinet}     &  \textbf{car} &    \textbf{chair}     &  \textbf{display}     &  \textbf{lamp}     &  \textbf{speaker} & \textbf{rifle}     &  \textbf{sofa}     &  \textbf{table}     &  \textbf{phone} & \textbf{vessel} & \textbf{mean}\\    
    \midrule
    \textbf{3D-R2N2}~\cite{choy20163d}  &  62.0 & 53.0 & 69.7 & 80.6 & 57.7 & 55.1 & 44.5 & 63.5 & 61.6 & 66.3 & 58.8 & 74.3 & 59.5 & 62.1  \\
    \textbf{Ours (w/o sym)} & 61.5 & 56.0  & 75.3  & 81.1  & 63.1  & 58.9  & 47.2  & 65.9  & 68.3  & 74.6  & 59.8  & 73.4  & 63.6  & 65.3  \\
    \textbf{Ours (w. sym)}  &  64.6 & 63.5 & 77.5 & 82.0 & 66.1 & 60.5 & 52.9 & 68.5 & 68.8 & 77.0 & 68.7 & 74.6 & 65.8 & 68.5  \\
    \bottomrule \\
  \end{tabular}}
\caption{\small{Mean Voxel IoU with 4 input views.}}
\tablelabel{mv3d}
%\vspace{-0.7cm}
\end{table}

\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{7pt}
\begin{table}[htb!]
\centering
\vspace{0pt}
\centering
\footnotesize
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{lccccccccccccc|c}
    \toprule
         &  \textbf{1 view}     &  \textbf{2 views}     &  \textbf{4 views}     &  \textbf{8 views}\\    
    \midrule
    \textbf{3D-R2N2}~\cite{choy20163d}  & 55.1 & 59.4 & 62.1 & -- \\
    \textbf{Ours (w/o sym)} & 55.2  & 61.5  & 65.3 & 65.9  \\
    \textbf{Ours (w. sym)}  & 58.2  & 65.7 & 68.5 & 69.1  \\
    \midrule
    \textbf{Ours (w. sym v2)}  & 57.0  & 64.1 & 67.7 & 68.6  \\
    \textbf{DnP + Fusion}  & 56.2  & 64.0 & 68.2 & 69.5  \\
    \midrule
    \textbf{LSM (GT pose)}  & 61.5  & 72.1 & 78.2 & -- \\
    \textbf{DnP (GT Pose)}  & 64.0 & 72.8 &  & 78.1  \\
    \midrule
    \textbf{Rendering} \\
    \textbf{Ours (w. sym v2)}  & 0.0480  & 0.0368 & 0.0316 & 0.0314  \\
    \textbf{DnP + Fusion}  & 0.0498  & 0.0384 & 0.0329 & 0.0319  \\    \bottomrule \\  \end{tabular}}
\caption{\small{Mean Voxel IoU across classes with variable number of input views during inference. Our model is always trained with 4 views at training.}}
\tablelabel{mv3dviews}
%\vspace{-0.7cm}
\end{table}

\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{7pt}
\begin{table}[htb!]
\centering
\vspace{0pt}
\centering
\footnotesize
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{lccccccccccccc|c}
    \toprule
         &  \textbf{1 view}     &  \textbf{2 views}     &  \textbf{4 views}     &  \textbf{8 views}\\    
    \midrule
    \textbf{3D-R2N2}~\cite{choy20163d}  & --  & --  & 62.0  & -- \\
    \textbf{Ours (w/o sym)} & 50.3  & 56.7  & 60.1 & 60.9 \\
    \textbf{Ours (w. sym)} & 54.8 & 61.3 & 64.6  & 65.6 \\
    \textbf{DnP + Fusion} & -- & 57.9 & 61.8 & 62.2  \\
    %\midrule
    %\textbf{DnP (GT pose) + Fusion} &  55.0  & 66.9 & 73.4  & 76.1 \\    \bottomrule \\
    \midrule
    \textbf{Rendering} \\
    \textbf{Ours (w. sym v2)} & 0.0478 (0.853) & 0.0386 (0.860)  & 0.0337 (0.865) & \\
    \textbf{DnP + Fusion}  & 0.0520 (0.851)  & 0.0420 (0.857) & 0.0361 (0.862) &  \\
    %\midrule
    %\textbf{DnP (GT pose) + Fusion}  & 0.0454 (0.856)  & 0.0322 (0.872) & 0.0246 (0.884) &  \\
    \bottomrule \\
    \end{tabular}}
\caption{\textbf{Results on data with camera translation.} \small{Mean Voxel IoU across classes with variable number of input views during inference. Our model is always trained with 4 views at training.}}
\tablelabel{mv3dviewstrans}
%\vspace{-0.7cm}
\end{table}
